How Do Large Language Models Understand Graph Patterns? A Benchmark for Graph Pattern Comprehension

Benchmarking the capabilities and limitations of large language models (LLMs) in graph-related tasks is becoming an increasingly popular and crucial area of research. Recent studies have shown that LLMs exhibit a preliminary ability to understand graph structures and node features. However, the potential of LLMs in graph pattern mining remains largely unexplored. This is a key component in fields such as computational chemistry, biology, and social network analysis. To bridge this gap, this work introduces a comprehensive benchmark to assess LLMs' capabilities in graph pattern tasks. We have developed a benchmark that evaluates whether LLMs can understand graph patterns based on either terminological or topological descriptions. Additionally, our benchmark tests the LLMs' capacity to autonomously discover graph patterns from data. The benchmark encompasses both synthetic and real datasets, and a variety of models, with a total of 11 tasks and 7 models. Our experimental framework is designed for easy expansion to accommodate new models and datasets. Our findings reveal that: (1) LLMs have preliminary abilities to understand graph patterns, with O1-mini outperforming in the majority of tasks; (2) Formatting input data to align with the knowledge acquired during pretraining can enhance performance; (3) The strategies employed by LLMs may differ from those used in conventional algorithms.

==> Sections/035_theory.tex <==
\section{Theoretical Insights of LLMs for Graphs}
In this section, we endeavor to develop the \textbf{minimum} theoretical results that can be used to develop insights for experiments. 

\textbf{Why not expressiveness?} The expressiveness is the most popular method to understand the reasoning abilities of LLMs \cite{feng2024towards,li2024chain,de2024simulation}. From the existing results, one can easily establish expressiveness results for LLM-based graph pattern recognition. One can first follow the proof of Theorem 1 in \cite{wu2024can} to show that LLMs have the capacity to simulate LOCAL algorithm (Computational model 2 in \cite{loukas2019graph}) when give adjacency list or edge list as input. Therefore, LLMs can perform graph pattern recognition as LOCAL algorithms can \cite{loukas2019graph}. It shows that there exists an LLMs that can perform graph pattern recognition. 

However, the expressiveness result provides limited insights for the experiments. Empirically, different prompts have different degree of success in graph reasoning tasks ({\color {red} An example}). However, the input graph format has no impact on the expressiveness. To provide insights, we should have more fine-grained results than expressiveness. 



\subsection{Algorithmic Alignment for LLMs}
Before the era of LLMs, researchers empirically observed that specialized network structures (e.g., GNNs) generalize better than less structured networks (e.g., MLPs) in reasoning tasks, although they have the same expressive power. Algorithmic alignment framework \cite{xu2019can} was proposed to address this issue. In LLMs, the Transformer architecture is fixed while the prompt is flexible. Therefore, we modify the algorthmic aligment framework from neural architecture to prompts such as input graph format. Next, we study how the prompt and graph reasoning task may interact, and possible implications for the performance. 

\textbf{Intuition.} The graph reasoning tasks can usually be computed with a reasoning algorithm. ({\color {red} An example}) Intuitively, a prompt may perform better if it let LLMs represent the underlying graph reasoning algorithm ``more easily''. Fig. illustrates this idea for the {\color {red} An example}


\textbf{Easiness of Learning.} Like the original algorithmic alignment paper \cite{xu2019can}, we formalize the easiness of learning via PAC framework and sample complexity. PAC learnability formalizes the \emph{easiness} via sample complexity, i.e., the number of training samples to ensure a low test error with high probability. It refers a learning algorithm $\mathcal{A}$ that, given training samples $\{x_i, y_i\}_{i=1}^M$ outputs a function $f=\mathcal{A}(\{x_i, y_i\}_{i=1}^M)$. The prompt influences the input format $x_i$, 


\textbf{The Interplay between Prompts and Tasks.}




==> Tables/application_detection.tex <==

\begin{table}[ht!]
  \centering
  \caption{Pattern Detection Result in real-world data.}
    \resizebox{\textwidth}{!}{\begin{tabular}{cc|ccc|ccc|ccc}
    \toprule
    \multicolumn{2}{c|}{Dataset} & \multicolumn{3}{c|}{Benzene} & \multicolumn{3}{c|}{Alkane-Carbonyl} & \multicolumn{3}{c}{Fluoride-Carbonyl} \\
    \multicolumn{2}{c|}{Model} & GPT-4 & GPT-4o & O1-mini & GPT-4 & GPT-4o & O1-mini & GPT-4 & GPT-4o & O1-mini \\
    \midrule
    \multirow{3}[1]{*}{node} & Accuracy & 0.88  & 0.71  & 0.88  & 0.63  & 0.65  & 0.69  & 0.65  & 0.59  & 0.65 \\
          & F1 & 0.89  & 0.78  & 0.89  & 0.46  & 0.49  & 0.51  & 0.51  & 0.52  & 0.52 \\
          & AUC   & 0.88  & 0.73  & 0.88  & 0.59  & 0.6   & 0.56  & 0.51  & 0.53  & 0.53 \\
          \midrule
          \multirow{3}[1]{*}{edge} & Accuracy & 0.82  & 0.71  & 0.88  & 0.53  & 0.63  & 0.71  & 0.64  & 0.58  & 0.66 \\
          & F1 & 0.83  & 0.75  & 0.89  & 0.49  & 0.52  & 0.58  & 0.53  & 0.52  & 0.51 \\
          & AUC   & 0.82  & 0.73  & 0.88  & 0.53  & 0.56  & 0.59  & 0.59  & 0.52  & 0.52 \\
    \bottomrule
    \end{tabular}}%
  \label{tab:app_detection}%
\end{table}%





% \begin{table}[htbp]
%   \centering
%   \small
%   \caption{Pattern Detection Result in real-world data.}
%     \begin{tabular}{cc|cccccc}
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}[1]{*}{Dataset}} & \multirow{2}[1]{*}{model} & \multicolumn{3}{c}{node} & \multicolumn{3}{c}{edge} \\
%           & \multicolumn{1}{c|}{} & Accuracy & F1 & AUC & Accuracy & F1 & AUC \\
%     \midrule
%     \multicolumn{1}{c}{\multirow{3}[2]{*}{benzene}} & GPT-4 & 0.88  & 0.89  & 0.88  & 0.82  & 0.83  & 0.82 \\
%           & GPT-4o & 0.71  & 0.78  & 0.73  & 0.71  & 0.75  & 0.73 \\
%           & O1-mini & 0.88  & 0.89  & 0.88  & 0.88  & 0.89  & 0.88 \\
%     \midrule
%     \multicolumn{1}{c}{\multirow{3}[2]{*}{alkane-carbon}} & GPT-4 & 0.63  & 0.46  & 0.59  & 0.53  & 0.49  & 0.53 \\
%           & GPT-4o & 0.65  & 0.49  & 0.6   & 0.63  & 0.52  & 0.56 \\
%           & O1-mini & 0.69  & 0.51  & 0.56  & 0.71  & 0.58  & 0.59 \\
%     \midrule
%     \multicolumn{1}{c}{\multirow{3}[2]{*}{fluoride-carbon}} & GPT-4 & 0.65  & 0.51  & 0.51  & 0.64  & 0.53  & 0.59 \\
%           & GPT-4o & 0.59  & 0.52  & 0.53  & 0.58  & 0.52  & 0.52 \\
%           & O1-mini & 0.65  & 0.52  & 0.53  & 0.66  & 0.51  & 0.52 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:app_detection}%
% \end{table}%



==> Tables/application_multiclass_results.tex <==

\begin{table}[ht!]
  \centering
  \small
  \caption{Result of multi-label classification tasks.}
    \resizebox{\textwidth}{!}{\begin{tabular}{c|rrrr|rrrr|rrrr}
    \toprule
    Dataset & \multicolumn{4}{c|}{ENZYMES}  & \multicolumn{4}{c|}{Fingerprint} & \multicolumn{4}{c}{IMDB-MULTI} \\
    Model & \multicolumn{2}{c}{GPT-4} & \multicolumn{2}{c|}{GPT-4o} & \multicolumn{2}{c}{GPT-4} & \multicolumn{2}{c|}{GPT-4o} & \multicolumn{2}{c}{GPT-4} & \multicolumn{2}{c}{GPT-4o} \\
    \midrule
    Method & \multicolumn{1}{l}{N.L.} & \multicolumn{1}{l}{E.L.} & \multicolumn{1}{l}{N.L.} & \multicolumn{1}{l|}{E.L.} & \multicolumn{1}{l}{N.L.} & \multicolumn{1}{l}{E.L.} & \multicolumn{1}{l}{N.L.} & \multicolumn{1}{l|}{E.L.} & \multicolumn{1}{l}{N.L.} & \multicolumn{1}{l}{E.L.} & \multicolumn{1}{l}{N.L.} & \multicolumn{1}{l}{E.L.} \\
    Accuracy & 0.40  & 0.38  & 0.40  & 0.35  & 0.36  & 0.36  & 0.35  & 0.34  & 0.33  & 0.35  & 0.34  & 0.35  \\
    \bottomrule
    \end{tabular}}%
  \label{tab:multi}%
\end{table}%

